Mental-LLM: Leveraging Large Language Models for Mental Health Prediction via Online Text Data

Advances in large language models (LLMs) have empowered a variety of applications. However, there is still a significant gap in research when it comes to understanding and enhancing the capabilities of LLMs in the field of mental health. In this work, we present a comprehensive evaluation of multiple LLMs on various mental health prediction tasks via online text data, including Alpaca, Alpaca-LoRA, FLAN-T5, GPT-3.5, and GPT-4. We conduct a broad range of experiments, covering zero-shot prompting, few-shot prompting, and instruction fine-tuning. The results indicate a promising yet limited performance of LLMs with zero-shot and few-shot prompt designs for mental health tasks. More importantly, our experiments show that instruction finetuning can significantly boost the performance of LLMs for all tasks simultaneously. Our best-finetuned models, Mental-Alpaca and Mental-FLAN-T5, outperform the best prompt design of GPT-3.5 (25 and 15 times bigger) by 10.9% on balanced accuracy and the best of GPT-4 (250 and 150 times bigger) by 4.8%. They further perform on par with the state-of-the-art task-specific language model. We also conduct an exploratory case study on LLMs' capability on mental health reasoning tasks, illustrating the promising capability of certain models such as GPT-4. We summarize our findings into a set of action guidelines for potential methods to enhance LLMs' capability for mental health tasks. Meanwhile, we also emphasize the important limitations before achieving deployability in real-world mental health settings, such as known racial and gender bias. We highlight the important ethical risks accompanying this line of research.

==> fig_tab_alg_/fig_dataset_distinguish.tex <==
\begin{figure}[b]
    \centering
    \includegraphics[width=1\columnwidth]{figures/results_dataset_distinguish_yweeklylevel.png}
    \caption{Results of The "Name-The-Dataset" Task using A Simple Random Forest Model. \review{Four colored lines indicate the accuracy of the four datasets, and the black line indicates the overall accuracy}. Error bar indicates the standard error. The same below.}
    \label{fig:dataset_distinguish}
\end{figure}

==> fig_tab_alg_/fig_dataset_person_distinguish.tex <==
\begin{figure}[b]
    \centering
    \begin{subfigure}[b]{.495\textwidth}
    \centering
    \includegraphics[width=1\columnwidth]{figures/results_dataset_distinguish_yweeklylevel.png}
    \caption{``Name-The-Dataset'' Task Results}
    \label{subfig:domain_distinguish:dataset_distinguish}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.495\textwidth}
    \centering
    \includegraphics[width=1\columnwidth]{figures/results_person_distinguish_yweeklylevel.png}
    \caption{``Distinguish-The-Person'' Task Results}
    \label{subfig:domain_distinguish:person_distinguish}
    \end{subfigure}
    \caption{\review{Results of Domain Classification Tasks using Simple Random Forest. \review{Four colored lines indicate the accuracy of the four datasets, and the black line indicates the overall accuracy}. Error bar indicates the standard error. The same below.}}
    \label{fig:domain_distinguish}
\end{figure}

==> fig_tab_alg_/fig_overview.tex <==
\begin{figure}[t]
    \vspace{-0.5cm}
    \centering
    \includegraphics[width=0.85\columnwidth]{figures/fig1-overview.png}
    \caption{Overview of The Contributions of This Work. We systematically evaluate cross-dataset generalizability of 19 algorithms: 9 prior behavior modeling algorithm for depression detection, 8 recent domain generalization algorithms, and 2 two new algorithms proposed in this paper. Our open-source platform GLOBEM consolidates these 19 algorithms and support using, developing, evaluating various algorithms.}
    \label{fig:overview}
    \vspace{-0.5cm}
\end{figure}

==> fig_tab_alg_/fig_person_distinguish.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{figures/results_person_distinguish_yweeklylevel.png}
    \caption{Results of The "Distinguish-The-Subject" Task using Another Simple Random Forest Model. \review{Four colored lines indicate the average classification accuracy of subjects in each of the four datasets, and the black line indicates the overall accuracy}.}
    \label{fig:person_distinguish}
\end{figure}

==> fig_tab_alg_/fig_platform_design.tex <==
\begin{figure}[b]
    \centering
    \includegraphics[width=1\columnwidth]{figures/platform_design.png}
    \caption{Design of The Benchmark Platform GLOBEM. It modularizes the pipeline and supports flexible adjustment of the existing algorithms and easy development of new algorithms.}
    \label{fig:platform}
\end{figure}

==> fig_tab_alg_/fig_reorder_design.tex <==
\begin{figure}[b]
    \centering
    \includegraphics[width=1\columnwidth]{figures/reorder_design.png}
    \caption{The Design of Reorder Compared to ERM. In addition the main behavior modeling task, Reorder further introduces a secondary task of solving a reorder puzzle to force the model to learn the continuity of behavior trajectory.}
    \label{fig:reorder_design}
\end{figure}

==> fig_tab_alg_/fig_reorder_more_experiment.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{.635\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{figures/results_allbutoneds_reorder_hyperparameter.png}
    \caption{Tuning of Hyper-parameters}
    \label{subfig:reorder_more_experiment:hyperparameter}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.355\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{figures/results_allbutoneds_ablation_study.png}
    \caption{Feature Ablation Study}
    \label{subfig:reorder_more_experiment:ablation}
    \end{subfigure}
    \caption{\review{Extra Experiments on \textit{Reorder} to Better Understanding the Model and Features. The experiments use the leave-one-dataset-out setup to ensure consistency. The dashed line indicates the performance of the best baseline models.}}
    \label{fig:reorder_more_experiment}
\end{figure}

==> fig_tab_alg_/fig_results_allbutoneds_allmethods_weekly.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{figures/results_allbutoneds_allmethods_weekly_pointplot.png}
    \caption{Model Performance of Predicting Bi-Weekly Depression Status across Datasets. The models are ranked based on the average results in Table~\ref{tab:results_allbutoneds_allmethods_weekly}. The dashed line indicates naive majority baseline. The same below.}
    \label{fig:results_allbutoneds_allmethods_weekly}
\end{figure}

==> fig_tab_alg_/fig_results_allbutoneds_allmethods_weekly_leak.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{figures/results_allbutoneds_allmethods_weekly_leak_pointplot.png}
    \caption{Model Performance of Predicting Bi-Weekly Depression Status across Datasets. Models are tested on one dataset after being trained on all other datasets with the optimal epoch numbers.}
    \label{fig:results_allbutoneds_allmethods_weekly_leak}
\end{figure}

==> fig_tab_alg_/fig_results_crossgroup_allmethods_weekly.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{figures/results_crossgroup_allmethods_weekly_pointplot_rocauc.png}
    \caption{\review{Model Performance of Predicting Bi-Weekly Depression Status across Institutions (left) and Years (middle, right) . Models are tested on the datasets of one year/institution after being trained on the other year/institution.}}
    \label{fig:results_crossgroup_allmethods_weekly}
\end{figure}

==> fig_tab_alg_/fig_single_feat_analysis.tex <==
\begin{figure}[b]
    \centering
    \begin{subfigure}[b]{.45\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{figures/singlefeat_significant_correlation_examples_lme.png}
    \caption{\review{Linear Mixed Model Coefficients of Example Features}}
    \label{subfig:sigle_feat_analysis:correlation}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.54\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{figures/singlefeat_pdf_examples.png}
    \caption{Distribution Comparison of Example Features}
    \label{subfig:sigle_feat_analysis:pdf}
    \end{subfigure}
    \caption{Features Analysis across All Datasets. (a) \review{Each data type's top features with consistent coefficients of linear mixed effect models between the feature value and depression labels across all datasets. Red indicates negative coefficients and blue indicates positive coefficients. Error bar indicates standard error.} (b) Example features' distribution across all datasets, which reveals how datasets can differ from each other. Datasets of the same institute are coded with closer colors. DS1 (green) and DS2 (blue) belong to the same institute, and DS3 (orange) and DS4 (red) belong to the other institute.}
    \label{fig:sigle_feat_analysis}
\end{figure}

==> fig_tab_alg_/tab_ablation_study.tex <==
% \renewcommand{\arraystretch}{1.3}
\begin{table}[!h]
\centering
\caption{Ablation Analysis on DS1 of Two Algorithms Developed on Overlapping Datasets. User set difference: consistent inclusion criteria cross all other algorithm \vs more strict data filtering criteria with fewer users; Evaluation difference: 20-fold cross validation \vs leave-one-user-out; Feature Difference: four feature types \vs additional location contexts, Bluetooth, WiFi, call, battery features.}
% \begin{minipage}[t]{0.48\textwidth}
% \resizebox{1\textwidth}{!}{
\begin{tabular}[t]{l|cc}

%%% Holder of the title columns %%%
% \multirow{2}{*}{\textbf{Model}} & \multicolumn{5}{c|}{\textbf{Balanced Accuracy}} & \multicolumn{5}{c}{\textbf{ROC AUC}}\\ \cline{2-11}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\hline \hline

\multirow{2}{*}{\textbf{Changes}} & \multicolumn{2}{c}{\textbf{Balanced Accuracy}}\\
& Xu \etal - Interpretable~\cite{xu_leveraging_2019} & Xu \etal - Personalized~\cite{xu_leveraging_2021}\\
\hline
Our Results & 0.722 & 0.738 \\
Remove User Set Difference & 0.719 & 0.748 \\
Remove Evaluation Difference & 0.749 & 0.742\\
Remove Feature Difference & 0.792 & 0.805 \\
\textit{Original Reported Results} & 0.806 & 0.819\\
\hline \hline
\end{tabular}
% }
\label{tab:ablation_study}
% \end{minipage}

% \vspace{0.1cm}
\end{table}
\renewcommand{\arraystretch}{1.0}

==> fig_tab_alg_/tab_demographics.tex <==
\renewcommand{\arraystretch}{1.3}
\begin{table}[b]
\centering
\caption{Basic Study Information and Participant Demographics of Four Datasets. Participants with less than 2 weekly EMAs or less than a quarter of their sensor data (\ie missing rate $>$ 75\%) were excluded from the dataset. In the ground truth row, the percentage in the parentheses indicates the proportion of participants having at least mild depressive symptoms based on the corresponding questionnaires. Gender acronym - F: Female, M: Male, NB: Non-binary. Racial acronym - A: Asian, B: Black or African American, H: Hispanic, N: American Indian/Alaska Native, PI: Pacific Islander, W: White, NA: Did not report. \& is used when participants reported more than one races.}
% \begin{minipage}[t]{0.1\textwidth}
\resizebox{1\textwidth}{!}{
\begin{tabular}{r|ll|ll}
\hline \hline
& \multicolumn{2}{c|}{\textbf{Institute1}} & \multicolumn{2}{c}{\textbf{Institute2}} \\ \cline{2-5}
& \makecell[c]{\textbf{Year1 - DS1}} & \makecell[c]{\textbf{Year2 - DS2}} & \makecell[c]{\textbf{Year1 - DS3}} & \makecell[c]{\textbf{Year2 - DS4}} \\
\hline
\addstackgap[20pt]{\textbf{Participants}}         & \makecell[l]{\text{ }\\- Total: 155\\ - Gender: F 107, M 48\\ - Race: A 82, B 5, H 9, N 4,\\PI 3,  W 50, A\&PI 2 \\ \text{ } \\ \text{ } \\ \text{ } } & \makecell[l]{\text{ }\\- Total: 218\\ - Gender: F 111, M 107\\ - Race: A 102, B 6, H 10, N 2, \\ PI 1, W 70, A\&B 1, A\&W 16, \\H\&W 2, B\&W 2, A\&H\&W 1,\\ B\&H\&W 1, H\&N\&W 1, NA 3 \\ - 23 also in Year1} & \makecell[l]{\text{ }\\- Total: 93\\ - Gender: F 65, M 27, NB 1\\  - Race: A 20, B 3, H 2, N 4, PI 1,\\W 52, B\&H 1, H\&W 5, NA 5\\ \text{ }\\ \text{ }\\ \text{ }}                                                                     & \makecell[l]{\text{ }\\- Total: 152\\ - Gender: F 101, M 49, NB 2\\ - Race: A 28, B 2, H 4, \\ N 4, W 100, B\&H 1, NA 13 \\ - 58 also in Year1\\ \text{ }\\ \text{ }} \\ % \hline
\addstackgap[15pt]{\textbf{Ground Truth}}         & \makecell[l]{- Weekly: Depression \& Affect  (44.4\%)\\ - End-term: BDI-II (35.4\%)}                                                   & \makecell[l]{- Weekly: PHQ-4 (50.3\%)\\ - End-term: BDI-II (42.9\%)}                            & \makecell[l]{- Weekly: PHQ-4 (35.9\%)\\ - End-term: PHQ-4 (42.4\%)}                                                                 & \makecell[l]{- Weekly: PHQ-4 (37.7\%)\\ - End-term: PHQ-4 (33.8\%)}\\ % \hline
\addstackgap[20pt]{\textbf{Sensor Data}} & \multicolumn{2}{l|}{\makecell[l]{- Overlap: Location, Phone Usage\\ - Compatible: Physical Activity (Fitbit), Sleep (Fitbit)\\ - Incompatible: Bluetooth, WiFi, Call, Battery}} & \multicolumn{2}{l}{\makecell[l]{- Overlap: Location, Phone Usage\\ - Compatible: Physical Activity (phone), Sleep (phone)\\ - Incompatible: Audio}} \\
\hline \hline
\end{tabular}
}
\label{tab:demographics}
\end{table}
\renewcommand{\arraystretch}{1.0}

==> fig_tab_alg_/tab_results_allbutoneds_allmethods_weekly.tex <==
% \renewcommand{\arraystretch}{1.3}
\begin{table}[t]
\centering
\caption{Model Performance of Predicting Weekly Depression Status across Datasets. Models are tested on one dataset after being trained on all other datasets. The Adv column indicates the advantage compared to the majority baseline. \review{$+$ or $-$ indicates the algorithm has at least one or no metric better than the baseline, with t-test statistical significance: $p< 0.1$\footnotesize{$_{\bullet}$}\normalsize{ (marginal significance), $<0.05^{*}$, $<0.01^{**}$, and $<0.001^{***}$.}}}
% \begin{minipage}[t]{0.48\textwidth}
\resizebox{1\textwidth}{!}{
\begin{tabular}[t]{l|ccccc|ccccc|l}

%%% Holder of the title columns %%%
% \multirow{2}{*}{\textbf{Model}} & \multicolumn{5}{c|}{\textbf{Balanced Accuracy}} & \multicolumn{5}{c}{\textbf{ROC AUC}}\\ \cline{2-11}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\hline \hline
\multirow{2}{*}{\textbf{Model}} & \multicolumn{5}{c|}{\textbf{ROC AUC}} & \multicolumn{5}{c|}{\textbf{Balanced Accuracy}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Adv}}} \\ \cline{2-11}
& \textbf{DS1} & \textbf{DS2} & \textbf{DS3} & \textbf{DS4} & \textbf{Avg} & \textbf{DS1} & \textbf{DS2} & \textbf{DS3} & \textbf{DS4} & \textbf{Avg} &\\
\hline
\textit{Majority Baseline}  & 0.500 & 0.500 & 0.500 & 0.500 & 0.500 & 0.500 & 0.500 & 0.500 & 0.500 & 0.500 & \\ \hdashline
Canzian \etal~\cite{canzian_trajectories_2015} & 0.490 & 0.493 & 0.457 & 0.537 & 0.494 & 0.499 & 0.500 & 0.500 & 0.500 & 0.500 & $-$ \\
Saeb \etal~\cite{saeb_mobile_2015} & 0.516 & 0.491 & 0.554 & 0.504 & 0.516 & 0.504 & 0.499 & 0.510 & 0.510 & 0.506 & $+$ \\
Farhan \etal~\cite{farhan_behavior_2016} & 0.509 & 0.472 & 0.483 & 0.493 & 0.489 & 0.517 & 0.489 & 0.509 & 0.489 & 0.501 & $+$ \\
Wahle \etal~\cite{wahle_mobile_2016} & 0.496 & 0.550 & 0.502 & 0.503 & 0.513 & 0.501 & 0.510 & 0.500 & 0.505 & 0.504 & $+$ \\
Lu \etal~\cite{lu_joint_2018} & 0.557 & 0.505 & 0.443 & 0.449 & 0.488 & 0.538 & 0.496 & 0.438 & 0.492 & 0.491 & $-$ \\
Wang \etal~\cite{wang_tracking_2018} & 0.536 & 0.539 & 0.500 & 0.500 & 0.519 & 0.501 & 0.502 & 0.500 & 0.500 & 0.501 & $+$ \\
Xu \etal - Interpretable~\cite{xu_leveraging_2019} & 0.457 & 0.507 & 0.461 & 0.496 & 0.480 & 0.501 & 0.498 & 0.478 & 0.502 & 0.495 & $-$ \\
Xu \etal - Personalized~\cite{xu_leveraging_2021} & 0.482 & 0.534 & 0.548 & 0.517 & 0.520 & 0.484 & 0.530 & 0.511 & 0.516 & 0.510 & $+$ \\
Chikersal \etal~\cite{chikersal_detecting_2021} & 0.590 & 0.525 & 0.526 & 0.523 & 0.541 & 0.545 & 0.503 & 0.523 & 0.508 & 0.520 & $+^{*}$ \\ \hdashline
ERM - 1D-CNN~\cite{vapnik1999overview} & 0.511 & 0.530 & 0.512 & 0.511 & 0.516 & 0.503 & 0.510 & 0.522 & 0.520 & 0.514 & $+^{*}$\\
ERM - 2D-CNN~\cite{vapnik1999overview} & 0.508 & 0.509 & 0.535 & 0.542 & 0.523 & 0.507 & 0.504 & 0.523 & 0.534 & 0.517 & $+^{*}$\\
ERM - LSTM~\cite{vapnik1999overview} & 0.518 & 0.516 & 0.536 & 0.511 & 0.520 & 0.511 & 0.502 & 0.528 & 0.502 & 0.511 & $+^{*}$\\
ERM - Transformer~\cite{vapnik1999overview} & 0.508 & 0.464 & 0.527 & 0.486 & 0.496 & 0.513 & 0.474 & 0.510 & 0.488 & 0.496 & $-$\\
ERM - Mixup~\cite{zhang_mixup_2018} & 0.512 & 0.522 & 0.513 & 0.520 & 0.517 & 0.517 & 0.505 & 0.519 & 0.513 & 0.514 & $+^{***}$\\
IRM~\cite{arjovsky_invariant_2020} & 0.546 & 0.514 & 0.518 & 0.507 & 0.521 & 0.532 & 0.513 & 0.524 & 0.510 & 0.520 & $+^{**}$ \\
DANN - Dataset as Domain~\cite{csurka_domain-adversarial_2017} & 0.501 & 0.510 & 0.465 & 0.506 & 0.496 & 0.499 & 0.500 & 0.500 & 0.500 & 0.500 & $-$ \\
DANN - Person as Domain~\cite{csurka_domain-adversarial_2017} & 0.512 & 0.511 & 0.470 & 0.507 & 0.500 & 0.500 & 0.500 & 0.500 & 0.500 & 0.500 & $-$ \\
CSD - Dataset as Domain~\cite{piratla_efficient_2020} & 0.519 & 0.530 & 0.516 & 0.504 & 0.517 & 0.517 & 0.530 & 0.504 & 0.494 & 0.511 & $+^{*}$\\
CSD - Person as Domain~\cite{piratla_efficient_2020} & 0.510 & 0.521 & 0.524 & 0.536 & 0.523 & 0.500 & 0.513 & 0.523 & 0.522 & 0.514 & $+^{**}$ \\
MLDG - Dataset as Domain~\cite{li_learning_2017} & 0.495 & 0.475 & 0.519 & 0.496 & 0.496 & 0.501 & 0.470 & 0.523 & 0.501 & 0.499 & $-$ \\
MLDG - Person as Domain~\cite{li_learning_2017} & 0.509 & 0.539 & 0.512 & 0.488 & 0.512 & 0.499 & 0.522 & 0.498 & 0.483 & 0.501 & $+$\\
MASF - Dataset as Domain~\cite{dou_domain_2019} & 0.505 & 0.514 & 0.506 & 0.522 & 0.512 & 0.496 & 0.499 & 0.509 & 0.499 & 0.501 & $+^{*}$\\
MASF - Person as Domain~\cite{dou_domain_2019} & 0.508 & 0.502 & 0.485 & 0.523 & 0.504 & 0.507 & 0.507 & 0.489 & 0.498 & 0.500 & $+$ \\
Siamese Network~\cite{koch_siamese_2015} & 0.512 & 0.509 & 0.488 & 0.508 & 0.504 & 0.512 & 0.509 & 0.488 & 0.508 & 0.504 & $+$ \\
Clustering & 0.522 & 0.502 & 0.497 & 0.521 & 0.511 & 0.518 & 0.505 & 0.499 & 0.517 & 0.510 & $+$\footnotesize{$_{\bullet}$}\\
\textbf{Reorder} & \textbf{0.584} & \textbf{0.588} & \textbf{0.580} & \textbf{0.548} & \textbf{0.575} & \textbf{0.570} & \textbf{0.546} & \textbf{0.558} & \textbf{0.535} & \textbf{0.552} & $+^{***}$\\
\hline \hline
\end{tabular}
}
\label{tab:results_allbutoneds_allmethods_weekly}
% \end{minipage}

% \vspace{0.1cm}
\end{table}
\renewcommand{\arraystretch}{1.0}

==> fig_tab_alg_/tab_results_allbutoneds_allmethods_weekly_balacc_rocauc.tex <==
% \renewcommand{\arraystretch}{1.3}
\begin{table}[b]
\centering
\caption{Model Performance of Predicting Weekly Depression Status across Datasets. Models are tested on one dataset after being trained on all other datasets. The Adv column indicates the advantage compared to the majority baseline. \review{$+$ or $-$ indicates the algorithm has at least one or no metric better than the baseline, with t-test statistical significance: $p< 0.1$\footnotesize{$^{\bullet}$}\normalsize{ (marginal significance), $<0.05^{*}$, $<0.01^{**}$, and $<0.001^{***}$.}}}
% \begin{minipage}[t]{0.48\textwidth}
\resizebox{1\textwidth}{!}{
\begin{tabular}[t]{l|ccccc|ccccc|l}

%%% Holder of the title columns %%%
% \multirow{2}{*}{\textbf{Model}} & \multicolumn{5}{c|}{\textbf{Balanced Accuracy}} & \multicolumn{5}{c}{\textbf{ROC AUC}}\\ \cline{2-11}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\hline \hline
\multirow{2}{*}{\textbf{Model}} & \multicolumn{5}{c|}{\textbf{Balanced Accuracy}} & \multicolumn{5}{c|}{\textbf{ROC AUC}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Adv}}} \\ \cline{2-11}
& \textbf{DS1} & \textbf{DS2} & \textbf{DS3} & \textbf{DS4} & \textbf{Avg} & \textbf{DS1} & \textbf{DS2} & \textbf{DS3} & \textbf{DS4} & \textbf{Avg} &\\
\hline
\textit{Majority Baseline}  & 0.500 & 0.500 & 0.500 & 0.500 & 0.500 & 0.500 & 0.500 & 0.500 & 0.500 & 0.500 & \\ \hdashline
Canzian \etal~\cite{canzian_trajectories_2015} & 0.499 & 0.500 & 0.500 & 0.500 & 0.500 & 0.490 & 0.493 & 0.457 & 0.537 & 0.494 & $-$ \\
Saeb \etal~\cite{saeb_mobile_2015} & 0.500 & 0.500 & 0.498 & 0.500 & 0.500 & 0.555 & 0.553 & 0.543 & 0.472 & 0.531 & $+$ \\
Farhan \etal~\cite{farhan_behavior_2016} & 0.517 & 0.489 & 0.509 & 0.489 & 0.501 & 0.509 & 0.472 & 0.483 & 0.493 & 0.489 & $+$ \\
Wahle \etal~\cite{wahle_mobile_2016} & 0.501 & 0.510 & 0.500 & 0.505 & 0.504 & 0.496 & 0.550 & 0.502 & 0.503 & 0.513 & $+$ \\
Lu \etal~\cite{lu_joint_2018} & 0.538 & 0.496 & 0.438 & 0.492 & 0.491 & 0.557 & 0.505 & 0.443 & 0.449 & 0.488 & $+$ \\
Wang \etal~\cite{wang_tracking_2018} & 0.501 & 0.502 & 0.500 & 0.500 & 0.501 & 0.536 & 0.539 & 0.500 & 0.500 & 0.519 & $+$ \\
Xu \etal - Interpretable~\cite{xu_leveraging_2019} & 0.501 & 0.498 & 0.478 & 0.502 & 0.495 & 0.457 & 0.507 & 0.461 & 0.496 & 0.480 & $+$ \\
Xu \etal - Personalized~\cite{xu_leveraging_2021} & 0.502 & 0.491 & 0.500 & 0.513 & 0.501 & 0.511 & 0.485 & 0.479 & 0.536 & 0.503 & $+$ \\
Chikersal \etal~\cite{chikersal_detecting_2021} & 0.545 & 0.503 & 0.523 & 0.508 & 0.520 & 0.590 & 0.525 & 0.526 & 0.523 & 0.541 & $+^{*}$ \\ \hdashline
ERM - 1D-CNN~\cite{vapnik1999overview} & 0.503 & 0.510 & 0.522 & 0.520 & 0.514 & 0.511 & 0.530 & 0.512 & 0.511 & 0.516 & $+^{*}$ \\
ERM - 2D-CNN~\cite{vapnik1999overview} & 0.507 & 0.504 & 0.523 & 0.534 & 0.517 & 0.508 & 0.509 & 0.535 & 0.542 & 0.523 & $+^{*}$\\
ERM - LSTM~\cite{vapnik1999overview} & 0.511 & 0.502 & 0.528 & 0.502 & 0.511 & 0.518 & 0.516 & 0.536 & 0.511 & 0.520 & $+^{*}$\\
ERM - Transformer~\cite{vapnik1999overview} & 0.513 & 0.474 & 0.510 & 0.488 & 0.496 & 0.508 & 0.464 & 0.527 & 0.486 & 0.496 & $-$\\
ERM - Mixup~\cite{zhang_mixup_2018} & 0.517 & 0.505 & 0.519 & 0.513 & 0.514 & 0.512 & 0.522 & 0.513 & 0.520 & 0.517 & $+^{***}$\\
IRM~\cite{arjovsky_invariant_2020} & 0.532 & 0.513 & 0.524 & 0.510 & 0.520 & 0.546 & 0.514 & 0.518 & 0.507 & 0.521 & $+^{**}$\\
DANN - Dataset as Domain~\cite{csurka_domain-adversarial_2017} & 0.499 & 0.500 & 0.500 & 0.500 & 0.500 & 0.501 & 0.510 & 0.465 & 0.506 & 0.496 & $-$\\
DANN - Person as Domain~\cite{csurka_domain-adversarial_2017} & 0.500 & 0.500 & 0.500 & 0.500 & 0.500 & 0.512 & 0.511 & 0.470 & 0.507 & 0.500 & $-$\\
CSD - Dataset as Domain~\cite{piratla_efficient_2020} & 0.517 & 0.530 & 0.504 & 0.494 & 0.511 & 0.519 & 0.530 & 0.516 & 0.504 & 0.517 & $+^{*}$\\
CSD - Person as Domain~\cite{piratla_efficient_2020} & 0.500 & 0.513 & 0.523 & 0.522 & 0.514 & 0.510 & 0.521 & 0.524 & 0.536 & 0.523 & $+^{**}$\\
MLDG - Dataset as Domain~\cite{li_learning_2017} & 0.501 & 0.470 & 0.523 & 0.501 & 0.499 & 0.495 & 0.475 & 0.519 & 0.496 & 0.496 & $-$\\
MLDG - Person as Domain~\cite{li_learning_2017} & 0.499 & 0.522 & 0.498 & 0.483 & 0.501 & 0.509 & 0.539 & 0.512 & 0.488 & 0.512  & $+$ \\
MASF - Dataset as Domain~\cite{dou_domain_2019} & 0.496 & 0.499 & 0.509 & 0.499 & 0.501 & 0.505 & 0.514 & 0.506 & 0.522 & 0.512 & $+^{*}$\\
MASF - Person as Domain~\cite{dou_domain_2019} & 0.507 & 0.507 & 0.489 & 0.498 & 0.500 & 0.508 & 0.502 & 0.485 & 0.523 & 0.504 & $+$\\
Siamese Network~\cite{koch_siamese_2015} & 0.512 & 0.509 & 0.488 & 0.508 & 0.504 & 0.512 & 0.509 & 0.488 & 0.508 & 0.504 & $+$\\ \hdashline
Clustering & 0.518 & 0.505 & 0.499 & 0.517 & 0.510 & 0.522 & 0.502 & 0.497 & 0.521 & 0.511 & $+$\footnotesize{$^{\bullet}$}\\
\textbf{Reorder} & \textbf{0.570} & \textbf{0.546} & \textbf{0.558} & \textbf{0.535} & \textbf{0.552} & \textbf{0.584} & \textbf{0.588} & \textbf{0.580} & \textbf{0.548} & \textbf{0.575} & $+^{***}$\\
\hline \hline
\end{tabular}
}
\label{tab:results_allbutoneds_allmethods_weekly}
% \end{minipage}

% \vspace{0.1cm}
\end{table}
\renewcommand{\arraystretch}{1.0}

==> fig_tab_alg_/tab_results_allbutoneds_allmethods_weekly_display_noreference.tex <==
% \renewcommand{\arraystretch}{1.3}
\begin{table}[b]
\centering
\caption{Model Performance of Predicting Weekly Depression Status across Datasets. Models are tested on one dataset after being trained on all other datasets.}
% \begin{minipage}[t]{0.48\textwidth}
\resizebox{1\textwidth}{!}{
\begin{tabular}[t]{l|ccccc|ccccc}

%%% Holder of the title columns %%%
% \multirow{2}{*}{\textbf{Model}} & \multicolumn{5}{c|}{\textbf{Balanced Accuracy}} & \multicolumn{5}{c}{\textbf{ROC AUC}}\\ \cline{2-11}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\hline \hline
\multirow{2}{*}{\textbf{Model}} & \multicolumn{5}{c|}{\textbf{Balanced Accuracy}} & \multicolumn{5}{c}{\textbf{ROC AUC}}\\ \cline{2-11}
& \textbf{Ins1 Y1} & \textbf{Ins1 Y2} & \textbf{Ins2 Y1} & \textbf{Ins2 Y2} & \textbf{Avg} & \textbf{Ins1 Y1} & \textbf{Ins1 Y2} & \textbf{Ins2 Y1} & \textbf{Ins2 Y2} & \textbf{Avg} \\
\hline
\textit{Majority Baseline}  & 0.500 & 0.500 & 0.500 & 0.500 & 0.500 & 0.500 & 0.500 & 0.500 & 0.500 & 0.500 \\ \hdashline
Canzian \etal & 0.499 & 0.500 & 0.500 & 0.500 & 0.500 & 0.490 & 0.493 & 0.457 & 0.537 & 0.494 \\
Saeb \etal & 0.500 & 0.500 & 0.498 & 0.500 & 0.500 & 0.555 & 0.553 & 0.543 & 0.472 & 0.531 \\
Farhan \etal & 0.517 & 0.489 & 0.509 & 0.489 & 0.501 & 0.509 & 0.472 & 0.483 & 0.493 & 0.489 \\
Wahle \etal & 0.501 & 0.510 & 0.500 & 0.505 & 0.504 & 0.496 & 0.550 & 0.502 & 0.503 & 0.513 \\
Lu \etal & 0.538 & 0.496 & 0.438 & 0.492 & 0.491 & 0.557 & 0.505 & 0.443 & 0.449 & 0.488 \\
Wang \etal & 0.501 & 0.502 & 0.500 & 0.500 & 0.501 & 0.536 & 0.539 & 0.500 & 0.500 & 0.519 \\
Xu \etal - Interpretable & 0.501 & 0.498 & 0.478 & 0.502 & 0.495 & 0.457 & 0.507 & 0.461 & 0.496 & 0.480 \\
Xu \etal - Personalized & 0.502 & 0.491 & 0.500 & 0.513 & 0.501 & 0.511 & 0.485 & 0.479 & 0.536 & 0.503 \\
Chikersal \etal & 0.545 & 0.503 & 0.523 & 0.508 & 0.520 & 0.590 & 0.525 & 0.526 & 0.523 & 0.541 \\ \hdashline
ERM - 1D-CNN & 0.503 & 0.510 & 0.522 & 0.520 & 0.514 & 0.511 & 0.530 & 0.512 & 0.511 & 0.516 \\
ERM - 2D-CNN & 0.507 & 0.504 & 0.523 & 0.534 & 0.517 & 0.508 & 0.509 & 0.535 & 0.542 & 0.523 \\
ERM - LSTM & 0.511 & 0.502 & 0.528 & 0.502 & 0.511 & 0.518 & 0.516 & 0.536 & 0.511 & 0.520 \\
ERM - Transformer & 0.513 & 0.474 & 0.510 & 0.488 & 0.496 & 0.508 & 0.464 & 0.527 & 0.486 & 0.496 \\
ERM - Mixup & 0.517 & 0.505 & 0.519 & 0.513 & 0.514 & 0.512 & 0.522 & 0.513 & 0.520 & 0.517 \\
IRM & 0.532 & 0.513 & 0.524 & 0.510 & 0.520 & 0.546 & 0.514 & 0.518 & 0.507 & 0.521 \\
DANN - Dataset as Domain & 0.499 & 0.500 & 0.500 & 0.500 & 0.500 & 0.501 & 0.510 & 0.465 & 0.506 & 0.496 \\
DANN - Person as Domain & 0.500 & 0.500 & 0.500 & 0.500 & 0.500 & 0.512 & 0.511 & 0.470 & 0.507 & 0.500 \\
CSD - Dataset as Domain & 0.517 & 0.530 & 0.504 & 0.494 & 0.511 & 0.519 & 0.530 & 0.516 & 0.504 & 0.517 \\
CSD - Person as Domain & 0.500 & 0.513 & 0.523 & 0.522 & 0.514 & 0.510 & 0.521 & 0.524 & 0.536 & 0.523 \\
MLDG - Dataset as Domain & 0.501 & 0.470 & 0.523 & 0.501 & 0.499 & 0.495 & 0.475 & 0.519 & 0.496 & 0.496 \\
MLDG - Person as Domain & 0.499 & 0.522 & 0.498 & 0.483 & 0.501 & 0.509 & 0.539 & 0.512 & 0.488 & 0.512 \\
MASF - Dataset as Domain & 0.496 & 0.499 & 0.509 & 0.499 & 0.501 & 0.505 & 0.514 & 0.506 & 0.522 & 0.512 \\
MASF - Person as Domain & 0.507 & 0.507 & 0.489 & 0.498 & 0.500 & 0.508 & 0.502 & 0.485 & 0.523 & 0.504 \\
Siamese Network & 0.512 & 0.509 & 0.488 & 0.508 & 0.504 & 0.512 & 0.509 & 0.488 & 0.508 & 0.504 \\
Clustering & 0.518 & 0.505 & 0.499 & 0.517 & 0.510 & 0.522 & 0.502 & 0.497 & 0.521 & 0.511 \\
Reorder & 0.570 & 0.546 & 0.558 & 0.535 & 0.552 & 0.584 & 0.588 & 0.580 & 0.548 & 0.575 \\
\hline \hline
\end{tabular}
}
\label{tab:results_allbutoneds_allmethods_weekly}
% \end{minipage}

% \vspace{0.1cm}
\end{table}
\renewcommand{\arraystretch}{1.0}

==> fig_tab_alg_/tab_results_multiple_setup.tex <==
% \renewcommand{\arraystretch}{1.3}
\begin{table}[t]
\centering
\caption{ROC AUC Summary of Multiple Evaluation Setups on The Weekly Depression Detection Task. The first column indicates the "optimal" setup. For traditional depression detection models, it is 20-fold cross validation on single dataset. For deep learning models, it is the best epoch selected based on the target dataset.}
\resizebox{1\textwidth}{!}{
\begin{tabular}[t]{L{4.8cm}|C{2.6cm}C{2.6cm}C{2cm}C{2cm}C{2cm}}
\hline \hline
\textbf{Model} & \makecell{\textbf{"Optimal" Setup} \\ \textbf{Single Dataset}} & \makecell{\textbf{Leave-One-}\\\textbf{Dataset-Out}} & \makecell{\textbf{Cross}\\\textbf{Institute}} & \makecell{\textbf{Cross Year}\\\text{ }} & \makecell{\textbf{Cross Year}\\\textbf{Overlapping}} \\
\hline
Canzian \etal~\cite{canzian_trajectories_2015} & 0.525 & 0.494 & 0.498 & 0.487 & 0.495 \\
Saeb \etal~\cite{saeb_mobile_2015} & 0.524 & 0.516 & 0.502 & \textbf{0.530} & 0.591 \\
Farhan \etal~\cite{farhan_behavior_2016} & 0.572 & 0.489 & 0.499 & 0.501 & 0.512 \\
Wahle \etal~\cite{wahle_mobile_2016} & 0.550 & 0.513 & 0.519 & 0.514 & 0.556 \\
Lu \etal~\cite{lu_joint_2018} & 0.542 & 0.488 & 0.500 & 0.479 & 0.528 \\
Wang \etal~\cite{wang_tracking_2018} & 0.527 & 0.519 & 0.522 & 0.498 & 0.525 \\
Xu \etal - Interpretable~\cite{xu_leveraging_2019} & 0.716 & 0.480 & 0.520 & 0.519 & 0.597 \\
Xu \etal - Personalized~\cite{xu_leveraging_2021} & 0.722 & 0.520 & \textbf{0.531} & 0.527 & 0.562 \\
Chikersal \etal~\cite{chikersal_detecting_2021} & \textbf{0.749} & \textbf{0.541} & 0.497 & 0.516 & \textbf{0.605} \\
\hline \hline
% \end{tabular}
% }
% \\
% \resizebox{1\textwidth}{!}{
% \begin{tabular}[t]{L{4.8cm}|C{2.5cm}C{2.5cm}C{2.5cm}C{2.5cm}C{2.5cm}}
% \hline \hline
\textbf{Model} & \makecell{\textbf{"Optimal" Setup} \\ \textbf{Best Epoch}} & \makecell{\textbf{Leave-One-}\\\textbf{Dataset-Out}} & \makecell{\textbf{Cross}\\\textbf{Institute}} & \makecell{\textbf{Cross Year}\\\text{ }} & \makecell{\textbf{Cross Year}\\\textbf{Overlapping}} \\
\hline
ERM - 1D-CNN~\cite{vapnik1999overview} & 0.531 & 0.516 & 0.498 & 0.520 & 0.517 \\
ERM - 2D-CNN~\cite{vapnik1999overview} & 0.550 & 0.523 & 0.504 & 0.504 & 0.539 \\
ERM - LSTM~\cite{vapnik1999overview} & 0.536 & 0.520 & 0.517 & 0.526 & 0.532 \\
ERM - Transformer~\cite{vapnik1999overview} & 0.523 & 0.496 & 0.510 & 0.496 & 0.509 \\
ERM - Mixup~\cite{zhang_mixup_2018} & 0.528 & 0.517 & 0.502 & 0.511 & 0.517 \\
IRM~\cite{arjovsky_invariant_2020} & 0.541 & 0.521 & 0.486 & 0.516 & 0.515 \\
DANN - Dataset as Domain~\cite{csurka_domain-adversarial_2017} & 0.499 & 0.496 & 0.498 & 0.505 & 0.537 \\
DANN - Person as Domain~\cite{csurka_domain-adversarial_2017} & 0.500 & 0.500 & 0.500 & 0.497 & 0.524 \\
CSD - Dataset as Domain~\cite{piratla_efficient_2020} & 0.522 & 0.517 & 0.506 & 0.526 & 0.565 \\
CSD - Person as Domain~\cite{piratla_efficient_2020} & 0.533 & 0.523 & 0.511 & 0.516 & 0.557 \\
MLDG - Dataset as Domain~\cite{li_learning_2017} & 0.508 & 0.496 & 0.501 & 0.499 & 0.534 \\
MLDG - Person as Domain~\cite{li_learning_2017} & 0.525 & 0.512 & 0.495 & 0.502 & 0.504 \\
MASF - Dataset as Domain~\cite{dou_domain_2019} & 0.501 & 0.512 & 0.505 & 0.507 & 0.509 \\
MASF - Person as Domain~\cite{dou_domain_2019} & 0.507 & 0.504 & 0.505 & 0.499 & 0.508 \\
Siamese Network~\cite{koch_siamese_2015} & 0.522 & 0.504 & 0.495 & 0.504 & 0.501 \\
Clustering & \textbf{0.582} & 0.511 & 0.516 & 0.495 & 0.481 \\
Reorder & 0.572 & \textbf{0.575} & \textbf{0.524} & \textbf{0.542} & \textbf{0.616} \\
\hline \hline
\end{tabular}
}
\label{tab:results_combined}
% \end{minipage}

% \vspace{0.1cm}
\end{table}
\renewcommand{\arraystretch}{1.0}

==> fig_tab_alg_/tab_results_multiple_setup_balacc.tex <==
% \renewcommand{\arraystretch}{1.3}
\begin{table}[t]
\centering
\caption{Balanced Accuracy Summary of Multiple Evaluation Setups on The Weekly Depression Detection Task. The first column indicates the "optimal" setup. For traditional depression detection models, it is 20-fold cross validation on single dataset. For deep learning models, it is the best epoch selected based on the target dataset.}
\resizebox{1\textwidth}{!}{
\begin{tabular}[t]{L{4.8cm}|C{2.6cm}C{2.6cm}C{2cm}C{2cm}C{2cm}}
\hline \hline
\textbf{Model} & \makecell{\textbf{"Optimal" Setup} \\ \textbf{Single Dataset}} & \makecell{\textbf{Leave-One-}\\\textbf{Dataset-Out}} & \makecell{\textbf{Cross}\\\textbf{Institute}} & \makecell{\textbf{Cross Year}\\\text{ }} & \makecell{\textbf{Cross Year}\\\textbf{Overlapping}} \\
\hline
Canzian \etal~\cite{canzian_trajectories_2015} & 0.525 & 0.500 & 0.498 & 0.499 & 0.518 \\
Saeb \etal~\cite{saeb_mobile_2015} & 0.522 & 0.500 & 0.500 & 0.500 & 0.556 \\
Farhan \etal~\cite{farhan_behavior_2016} & 0.572 & 0.501 & 0.\textbf{510} & 0.505 & 0.492 \\
Wahle \etal~\cite{wahle_mobile_2016} & 0.550 & 0.504 & 0.500 & 0.500 & 0.499 \\
Lu \etal~\cite{lu_joint_2018} & 0.542 & 0.491 & 0.506 & 0.491 & 0.521 \\
Wang \etal~\cite{wang_tracking_2018} & 0.527 & 0.501 & 0.499 & 0.500 & 0.525 \\
Xu \etal - Interpretable~\cite{xu_leveraging_2019} & 0.716 & 0.495 & 0.488 & 0.515 & \textbf{0.581} \\
Xu \etal - Personalized~\cite{xu_leveraging_2021} & 0.733 & 0.501 & 0.506 & \textbf{0.526} & 0.536 \\
Chikersal \etal~\cite{chikersal_detecting_2021} & \textbf{0.749} & \textbf{0.520} & 0.495 & 0.505 & 0.577 \\
\hline \hline
% \end{tabular}
% }
% \\
% \resizebox{1\textwidth}{!}{
% \begin{tabular}[t]{L{4.8cm}|C{2.5cm}C{2.5cm}C{2.5cm}C{2.5cm}C{2.5cm}}
% \hline \hline
\textbf{Model} & \makecell{\textbf{"Optimal" Setup} \\ \textbf{Best Epoch}} & \makecell{\textbf{Leave-One-}\\\textbf{Dataset-Out}} & \makecell{\textbf{Cross}\\\textbf{Institute}} & \makecell{\textbf{Cross Year}\\\text{ }} & \makecell{\textbf{Cross Year}\\\textbf{Overlapping}} \\
\hline
ERM - 1dCNN~\cite{vapnik1999overview} & 0.536 & 0.514 & 0.501 & 0.511 & 0.508 \\
ERM - 2dCNN~\cite{vapnik1999overview} & 0.541 & 0.517 & 0.499 & 0.503 & 0.532 \\
ERM - LSTM~\cite{vapnik1999overview} & 0.531 & 0.511 & 0.507 & 0.520 & 0.531 \\
ERM - Transformer~\cite{vapnik1999overview} & 0.521 & 0.496 & 0.505 & 0.496 & 0.501 \\
ERM - Mixup~\cite{zhang_mixup_2018} & 0.531 & 0.514 & 0.501 & 0.506 & 0.508 \\
IRM~\cite{arjovsky_invariant_2020} & 0.535 & 0.520 & 0.494 & 0.514 & 0.517 \\
DANN - Dataset as Domain~\cite{csurka_domain-adversarial_2017} & 0.500 & 0.500 & 0.500 & 0.500 & 0.525 \\
DANN - Person as Domain~\cite{csurka_domain-adversarial_2017} & 0.500 & 0.500 & 0.500 & 0.500 & 0.511 \\
CSD - Dataset as Domain~\cite{piratla_efficient_2020} & 0.519 & 0.511 & 0.505 & 0.515 & 0.553 \\
CSD - Person as Domain~\cite{piratla_efficient_2020} & 0.534 & 0.514 & 0.513 & 0.506 & 0.544 \\
MLDG - Dataset as Domain~\cite{li_learning_2017} & 0.516 & 0.499 & 0.500 & 0.495 & 0.522 \\
MLDG - Person as Domain~\cite{li_learning_2017} & 0.524 & 0.501 & 0.495 & 0.502 & 0.505 \\
MASF - Dataset as Domain~\cite{dou_domain_2019} & 0.508 & 0.501 & 0.502 & 0.500 & 0.522 \\
MASF - Person as Domain~\cite{dou_domain_2019} & 0.509 & 0.500 & 0.506 & 0.499 & 0.514 \\
Siamese Network~\cite{koch_siamese_2015} & 0.522 & 0.504 & 0.495 & 0.504 & 0.501 \\
Clustering & \textbf{0.595} & 0.510 & 0.515 & 0.492 & 0.483 \\
Reorder & 0.556 & \textbf{0.552} & \textbf{0.519} & \textbf{0.528} & \textbf{0.596} \\
\hline \hline
\end{tabular}
}
\label{tab:results_combined}
% \end{minipage}

% \vspace{0.1cm}
\end{table}
\renewcommand{\arraystretch}{1.0}

==> fig_tab_alg_/tab_results_oneds_existing_endterm_weekly.tex <==
% % \renewcommand{\arraystretch}{1.3}
% \begin{table}[b]
% \centering
% \begin{minipage}[t]{0.48\textwidth}
% \resizebox{1\textwidth}{!}{
% \begin{tabular}[t]{l|ccccc}
% \hline \hline
% \textbf{Model} & \textbf{UW-1} & \textbf{UW-2} & \textbf{DC-1} & \textbf{DC-2} & \textbf{Avg} \\
% \hline
% Canzian \etal~\cite{canzian_trajectories_2015} & 0.513 & 0.534 & 0.579 & 0.500 & 0.532 \\
% Saeb \etal~\cite{saeb_mobile_2015} & 0.544 & 0.503 & 0.500 & 0.494 & 0.510 \\
% Farhan \etal~\cite{farhan_behavior_2016} & 0.531 & 0.605 & 0.462 & 0.621 & 0.554 \\
% Wahle \etal~\cite{wahle_mobile_2016} & 0.487 & 0.562 & 0.500 & 0.590 & 0.535 \\
% Lu \etal~\cite{lu_joint_2018} & 0.506 & 0.533 & 0.414 & 0.610 & 0.516 \\
% Wang \etal~\cite{wang_tracking_2018} & 0.548 & 0.500 & 0.500 & 0.496 & 0.511 \\
% Xu \etal - Interpretable~\cite{xu_leveraging_2019} & 0.625 & 0.676 & 0.677 & 0.580 & 0.639 \\
% Xu \etal - Personalized~\cite{xu_leveraging_2021} & 0.673 & 0.605 & 0.633 & 0.612 & 0.631 \\
% Chikersal \etal~\cite{chikersal_detecting_2021} & 0.702 & 0.758 & 0.797 & 0.626 & 0.721 \\
% \hline \hline
% \end{tabular}}
% \caption{Balanced Accuracy of Predicting End-of-term Depression Status within Dataset. Models are evaluated by 5-fold cross-validation within each of the four datasets.}
% \label{tab:results_oneds_existing_endterm}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.48\textwidth}
% \resizebox{1\textwidth}{!}{
% \begin{tabular}[t]{l|ccccc}
% \hline \hline
% \textbf{Model} & \textbf{UW-1} & \textbf{UW-2} & \textbf{DC-1} & \textbf{DC-2} & \textbf{Avg} \\
% \hline
% Canzian \etal~\cite{canzian_trajectories_2015} & 0.512 & 0.500 & 0.495 & 0.501 & 0.502 \\
% Saeb \etal~\cite{saeb_mobile_2015} & 0.514 & 0.538 & 0.497 & 0.508 & 0.515 \\
% Farhan \etal~\cite{farhan_behavior_2016} & 0.524 & 0.507 & 0.494 & 0.501 & 0.506 \\
% Wahle \etal~\cite{wahle_mobile_2016} & 0.526 & 0.523 & 0.523 & 0.500 & 0.518 \\
% Lu \etal~\cite{lu_joint_2018} & 0.523 & 0.523 & 0.473 & 0.552 & 0.518 \\
% Wang \etal~\cite{wang_tracking_2018} & 0.552 & 0.500 & 0.500 & 0.500 & 0.513 \\
% Xu \etal - Interpretable~\cite{xu_leveraging_2019} & 0.598 & 0.551 & 0.604 & 0.561 & 0.578 \\
% Xu \etal - Personalized~\cite{xu_leveraging_2021} & 0.557 & 0.543 & 0.536 & 0.500 & 0.534 \\
% Chikersal \etal~\cite{chikersal_detecting_2021} & 0.602 & 0.591 & 0.598 & 0.562 & 0.588 \\
% \hline \hline
% \end{tabular}}
% \caption{Balanced Accuracy of Predicting Bi-Weekly Depression Status within Dataset. Models are evaluated by 5-fold cross-validation within each of the four datasets.}
% \label{tab:results_oneds_existing_weekly}
% \end{minipage}

% % \vspace{0.1cm}
% \end{table}
% \renewcommand{\arraystretch}{1.0}


% \renewcommand{\arraystretch}{1.3}
\begin{table}[b]
\centering
\caption{Balanced Accuracy of Predicting End-of-term or Weekly Depression Status. Models are evaluated by 5-fold cross-validation within each of the four datasets. The "Prior Work" columns show the performance contrast between the reported results in prior literature (evaluated on their own datasets) and the results on our datasets. $^{+}$/$^{++}$ means the literature only reported F1-score/ROC AUC, which was usually close to balanced accuracy.
}
% \begin{minipage}[t]{0.1\textwidth}
\resizebox{1\textwidth}{!}{
\begin{tabular}[t]{l|cccccc|cccccc}
\hline \hline
\multirow{2}{*}{\textbf{Model}} & \multicolumn{6}{c|}{\textbf{Task1: End-of-Term Depression Detection}} & \multicolumn{6}{c}{\textbf{Task2: Weekly Depression Detection}}\\ \cline{2-13}
& \textbf{DS1} & \textbf{DS2} & \textbf{DS3} & \textbf{DS4} & \textbf{Avg} & \textit{Prior Work} & \textbf{DS1} & \textbf{DS2} & \textbf{DS3} & \textbf{DS4} & \textbf{Avg} & \textit{Prior Work} \\
\hline
\textit{Majority Baseline} & 0.500 & 0.500 & 0.500 & 0.500 & 0.500 & - & 0.500 & 0.500 & 0.500 & 0.500 & 0.500 & - \\ \hdashline
Canzian \etal~\cite{canzian_trajectories_2015} & 0.559 & 0.516 & 0.526 & 0.500 & 0.525 & - & 0.512 & 0.497 & 0.512 & 0.500 & 0.505 & \textit{0.760} \\
Saeb \etal~\cite{saeb_mobile_2015} & 0.539 & 0.508 & 0.562 & 0.480 & 0.522 & \textit{0.791} & 0.496 & 0.549 & 0.508 & 0.506 & 0.515 & - \\
Farhan \etal~\cite{farhan_behavior_2016} & 0.552 & 0.609 & 0.505 & 0.620 & 0.572 & \textit{0.855} & 0.519 & 0.515 & 0.519 & 0.513 & 0.517 & - \\
Wahle \etal~\cite{wahle_mobile_2016} & 0.526 & 0.527 & 0.562 & 0.583 & 0.550 & - & 0.514 & 0.530 & 0.519 & 0.503 & 0.516 & \textit{0.616} \\
Lu \etal~\cite{lu_joint_2018} & 0.574 & 0.558 & 0.403 & 0.634 & 0.542 & - & 0.531 & 0.499 & 0.482 & 0.534 & 0.511 & \textit{0.770}$^{+}$ \\
Wang \etal~\cite{wang_tracking_2018} & 0.566 & 0.500 & 0.537 & 0.503 & 0.527 & - & 0.534 & 0.500 & 0.512 & 0.500 & 0.512 & \textit{0.809}$^{++}$ \\
Xu \etal - Interpretable~\cite{xu_leveraging_2019} & 0.722 & 0.623 & 0.815 & 0.706 & 0.716 & \textit{0.806} & 0.533 & 0.576 & 0.677 & 0.553 & 0.585 & - \\
Xu \etal - Personalized~\cite{xu_leveraging_2021} & 0.723 & 0.699 & 0.818 & 0.649 & 0.722 & \textit{0.819} & 0.568 & 0.562 & 0.614 & 0.572 & 0.579 & - \\
Chikersal \etal~\cite{chikersal_detecting_2021} & 0.728 & 0.776 & 0.795 & 0.698 & 0.749 & \textit{0.816} & 0.615 & 0.613 & 0.595 & 0.551 & 0.593 & - \\
\hline \hline
\end{tabular}
}
\label{tab:results_oneds_existing_endterm_weekly}
% \end{minipage}
% \vspace{0.1cm}
\end{table}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.90\columnwidth]{figures/performance_gap.png}
%     \caption{The Performance Gap between Model Results on Our Datasets \vs Reported Results in Prior Work, highlighting the results in Table~\ref{tab:results_oneds_existing_endterm_weekly}. The dashed line indicates naive majority baseline.
%     }
%     \label{fig:performance_gap}
% \end{figure}

\renewcommand{\arraystretch}{1.0}

==> fig_tab_alg_/tab_results_oneds_existing_endterm_weekly_fig.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.90\columnwidth]{figures/performance_gap.png}
    \caption{The Performance Gap between Model Results on Our Datasets \vs Reported Results in Prior Work, highlighting the results in Table~\ref{tab:results_oneds_existing_endterm_weekly}. The dashed line indicates naive majority baseline.
    }
    \label{fig:performance_gap}
\end{figure}
